Stopping Criterion Design for Recursive Bayesian Classification: Analysis and Decision Geometry

Systems that are based on recursive Bayesian updates for classification limit the cost of evidence collection through certain stopping/termination criteria and accordingly enforce decision making. Conventionally, two termination criteria based on pre-defined thresholds over (i) the maximum of the state posterior distribution; and (ii) the state posterior uncertainty are commonly used. In this paper, we propose a geometric interpretation over the state posterior progression and accordingly we provide a point-by-point analysis over the disadvantages of using such conventional termination criteria. For example, through the proposed geometric interpretation we show that confidence thresholds defined over maximum of the state posteriors suffer from stiffness that results in unnecessary evidence collection whereas uncertainty based thresholding methods are fragile to number of categories and terminate prematurely if some state candidates are already discovered to be unfavorable. Moreover, both types of termination methods neglect the evolution of posterior updates. We then propose a new stopping/termination criterion with a geometrical insight to overcome the limitations of these conventional methods and provide a comparison in terms of decision accuracy and speed. We validate our claims using simulations and using real experimental data obtained through a brain computer interfaced typing system.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> fig/tables/20191209_10522.tex <==
% 20191209_152513
\begin{table*}[t!]
%\small\addtolength{\tabcolsep}{-1pt}
\caption{\label{tab:acc_fixed_mean_1Q} Accuracy and number of recursions performed statistics for all methods presented in the paper using the setting in \cite{tsiligkaridis2014collaborative}. The evidence distributions are selected as 1D Gaussian distributions with means $\lbrace0,3 \rbrace$} and standard deviations $\lbrace 1, 3-\delta_\sigma \rbrace$ respectively.
{\def\arraystretch{1.5}\tabcolsep=3.5pt
\begin{center}
\tiny
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
& & \multicolumn{20}{c}{$3- \delta_\sigma$} \\
\cline{3-22}
&method &3 &2.9 &2.8 &2.7 &2.6 &2.5 &2.4 &2.3 &2.2 &2.1 &2 &1.9 &1.8 &1.7 &1.8 &1.7 &1.6 &1.5 &1.4 &1.3\\
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Accuracy}}} &M1 & 0.92 & 0.92 & 0.92 & 0.91 & 0.92 & 0.91 & 0.89 & 0.93 & 0.92 & 0.94 & 0.92 & 0.92 & 0.95 & 0.96 & 0.95 & 0.97 & 0.96 & 0.97 & 0.97 & 0.98\\
&M2 & 0.92 & 0.94 & 0.92 & 0.92 & 0.91 & 0.95 & 0.93 & 0.95 & 0.94 & 0.95 & 0.96 & 0.94 & 0.96 & 0.97 & 0.97 & 0.98 & 0.97 & 0.99 & 0.98 & 0.98\\
&M3 & 0.92 & 0.94 & 0.92 & 0.92 & 0.91 & 0.95 & 0.93 & 0.95 & 0.94 & 0.95 & 0.96 & 0.94 & 0.96 & 0.97 & 0.97 & 0.98 & 0.97 & 0.98 & 0.98 & 0.98\\
&M4 & 0.94 & 0.95 & 0.94 & 0.91 & 0.92 & 0.95 & 0.93 & 0.93 & 0.92 & 0.95 & 0.93 & 0.92 & 0.94 & 0.95 & 0.94 & 0.95 & 0.94 & 0.96 & 0.95 & 0.97\\
&M5 & 0.93 & 0.94 & 0.93 & 0.91 & 0.91 & 0.94 & 0.91 & 0.92 & 0.92 & 0.94 & 0.91 & 0.89 & 0.89 & 0.90 & 0.89 & 0.90 & 0.89 & 0.88 & 0.88 & 0.86\\
&M6 & 0.93 & 0.93 & 0.91 & 0.88 & 0.88 & 0.86 & 0.83 & 0.82 & 0.79 & 0.74 & 0.69 & 0.65 & 0.61 & 0.56 & 0.50 & 0.48 & 0.41 & 0.35 & 0.35 & 0.36\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Mean rec.}}} &M1 & 8.98 & 8.20 & 7.47 & 7.05 & 6.45 & 6.03 & 5.70 & 5.38 & 5.45 & 5.14 & 5.03 & 4.80 & 4.59 & 4.47 & 4.38 & 4.23 & 4.15 & 4.18 & 4.03 & 3.98\\
&M2 & 10.71 & 9.89 & 8.62 & 8.21 & 7.54 & 6.88 & 6.53 & 6.09 & 6.10 & 5.65 & 5.51 & 5.22 & 5.03 & 4.87 & 4.72 & 4.53 & 4.46 & 4.44 & 4.26 & 4.19\\
&M3 & 10.68 & 9.85 & 8.55 & 8.20 & 7.52 & 6.87 & 6.50 & 6.06 & 6.08 & 5.63 & 5.50 & 5.20 & 5.00 & 4.85 & 4.71 & 4.50 & 4.43 & 4.42 & 4.23 & 4.16\\
&M4 & 10.34 & 9.48 & 8.28 & 7.92 & 7.18 & 6.63 & 6.14 & 5.75 & 5.74 & 5.37 & 5.23 & 4.95 & 4.73 & 4.58 & 4.46 & 4.24 & 4.12 & 4.17 & 3.98 & 3.95\\
&M5 & 10.05 & 9.12 & 8.07 & 7.52 & 6.84 & 6.31 & 5.89 & 5.47 & 5.51 & 5.13 & 5.00 & 4.67 & 4.42 & 4.31 & 4.19 & 4.00 & 3.85 & 3.81 & 3.65 & 3.55\\
&M6 & 9.45 & 8.49 & 7.46 & 6.89 & 6.10 & 5.76 & 5.19 & 4.82 & 4.73 & 4.17 & 3.90 & 3.70 & 3.37 & 3.13 & 2.96 & 2.82 & 2.61 & 2.50 & 2.34 & 2.26\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Std. rec.}}} &M1 & 4.45 & 3.68 & 3.24 & 2.91 & 2.36 & 2.16 & 1.99 & 1.63 & 1.74 & 1.56 & 1.58 & 1.27 & 1.17 & 1.10 & 1.05 & 0.85 & 0.83 & 0.83 & 0.73 & 0.67\\
&M2 & 5.14 & 4.84 & 3.54 & 3.63 & 3.13 & 2.40 & 2.38 & 1.96 & 2.11 & 1.61 & 1.68 & 1.32 & 1.23 & 1.13 & 1.05 & 0.88 & 0.86 & 0.83 & 0.77 & 0.67\\
&M3 & 5.08 & 4.82 & 3.38 & 3.63 & 3.10 & 2.38 & 2.38 & 1.95 & 2.11 & 1.61 & 1.68 & 1.31 & 1.22 & 1.14 & 1.05 & 0.87 & 0.85 & 0.83 & 0.75 & 0.66\\
&M4 & 4.91 & 4.35 & 3.31 & 3.49 & 2.64 & 2.28 & 2.03 & 1.80 & 1.89 & 1.57 & 1.58 & 1.29 & 1.22 & 1.10 & 1.04 & 0.84 & 0.75 & 0.80 & 0.64 & 0.62\\
&M5 & 4.91 & 4.09 & 3.27 & 3.17 & 2.47 & 2.14 & 1.99 & 1.69 & 1.90 & 1.54 & 1.57 & 1.24 & 1.12 & 1.03 & 1.00 & 0.78 & 0.73 & 0.74 & 0.63 & 0.62\\
&M6 & 4.62 & 3.68 & 3.22 & 2.88 & 2.21 & 2.09 & 1.89 & 1.58 & 1.74 & 1.23 & 1.22 & 1.00 & 0.84 & 0.72 & 0.58 & 0.57 & 0.54 & 0.53 & 0.47 & 0.44\\
\hline
\end{tabular}
\end{center}
}
\end{table*}
%

==> fig/tables/20191209_11110.tex <==
%
\begin{table*}[t!]
%\small\addtolength{\tabcolsep}{-1pt}
\caption{\label{tab:acc_unit_var_10Q} Accuracy and number of recursions performed statistics for all methods presented in the paper using the setting in \cite{tsiligkaridis2014collaborative}. The evidence distributions are selected as 1D Gaussian distributions with unit variance. Evidence measurement performance is measured with the distance between means of the distributions. Proposed $(T)$ \textbf{(M1)} achieves higher accuracy with lower number of recursions on average with lesser variance.}
{\def\arraystretch{1.5}\tabcolsep=3.5pt
\begin{center}
\tiny
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
& & \multicolumn{20}{c}{$\delta_\text{means}$} \\
\cline{3-22}
&method &2.5 &2.6 &2.7 &2.8 &2.9 &3 &3.1 &3.2 &3.3 &3.4 &3.5 &3.6 &3.7 &3.8 &3.9 &4 &4.1 &4.2 &4.3 &4.4\\
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Accuracy}}} &M1 & 0.83 & 0.89 & 0.91 & 0.94 & 0.95 & 0.97 & 0.98 & 0.96 & 0.95 & 0.96 & 0.95 & 0.95 & 0.98 & 0.97 & 0.97 & 0.97 & 0.96 & 0.96 & 0.97 & 0.96\\
&M2 & 0.71 & 0.77 & 0.80 & 0.83 & 0.86 & 0.91 & 0.92 & 0.89 & 0.90 & 0.91 & 0.89 & 0.92 & 0.92 & 0.94 & 0.95 & 0.96 & 0.94 & 0.95 & 0.97 & 0.96\\
&M3 & 0.71 & 0.77 & 0.80 & 0.83 & 0.86 & 0.91 & 0.92 & 0.89 & 0.89 & 0.92 & 0.89 & 0.92 & 0.93 & 0.94 & 0.95 & 0.96 & 0.94 & 0.95 & 0.97 & 0.96\\
&M4 & 0.74 & 0.80 & 0.83 & 0.87 & 0.89 & 0.92 & 0.92 & 0.91 & 0.91 & 0.93 & 0.91 & 0.93 & 0.94 & 0.95 & 0.95 & 0.96 & 0.95 & 0.95 & 0.96 & 0.94\\
&M5 & 0.75 & 0.82 & 0.86 & 0.89 & 0.91 & 0.92 & 0.93 & 0.92 & 0.93 & 0.94 & 0.93 & 0.94 & 0.96 & 0.96 & 0.94 & 0.93 & 0.91 & 0.87 & 0.83 & 0.77\\
&M6 & 0.80 & 0.88 & 0.92 & 0.94 & 0.96 & 0.98 & 0.99 & 0.96 & 0.93 & 0.92 & 0.79 & 0.70 & 0.59 & 0.48 & 0.39 & 0.35 & 0.32 & 0.29 & 0.22 & 0.23\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Mean rec.}}} &M1 & 59.00 & 55.48 & 50.79 & 45.62 & 42.17 & 40.86 & 36.19 & 34.70 & 34.21 & 31.88 & 31.39 & 30.32 & 28.62 & 28.14 & 27.99 & 26.91 & 26.44 & 25.88 & 25.93 & 25.45\\
&M2 & 67.06 & 61.31 & 58.48 & 52.09 & 48.48 & 46.37 & 41.34 & 40.32 & 38.92 & 36.72 & 36.42 & 34.19 & 31.64 & 30.06 & 30.42 & 28.86 & 27.79 & 27.40 & 27.11 & 26.70\\
&M3 & 67.06 & 61.23 & 58.31 & 52.04 & 48.48 & 46.36 & 41.12 & 40.02 & 38.90 & 36.63 & 36.41 & 34.14 & 31.60 & 30.05 & 30.40 & 28.82 & 27.75 & 27.33 & 27.09 & 26.66\\
&M4 & 66.03 & 60.02 & 57.01 & 50.72 & 46.92 & 44.92 & 39.72 & 38.54 & 37.78 & 35.29 & 34.60 & 32.90 & 30.29 & 29.24 & 29.71 & 27.64 & 27.19 & 26.53 & 26.38 & 25.95\\
&M5 & 64.45 & 59.35 & 55.45 & 49.10 & 46.30 & 44.13 & 39.04 & 37.18 & 36.50 & 33.48 & 32.92 & 30.94 & 29.22 & 28.33 & 28.25 & 26.76 & 26.11 & 25.30 & 25.07 & 24.30\\
&M6 & 63.07 & 57.75 & 52.97 & 47.19 & 43.04 & 41.45 & 36.01 & 34.05 & 32.62 & 30.13 & 27.36 & 25.41 & 23.06 & 21.39 & 20.05 & 18.75 & 17.30 & 16.65 & 15.95 & 15.52\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Std. rec.}}} &M1 & 27.67 & 25.74 & 25.02 & 22.07 & 20.57 & 19.29 & 17.19 & 14.98 & 15.41 & 13.47 & 12.92 & 11.96 & 10.35 & 9.77 & 8.92 & 8.51 & 8.56 & 7.53 & 7.94 & 6.86\\
&M2 & 27.98 & 26.68 & 27.27 & 24.93 & 23.82 & 22.70 & 20.81 & 20.07 & 19.07 & 18.34 & 18.01 & 16.60 & 13.59 & 11.07 & 11.06 & 10.27 & 8.96 & 8.34 & 8.22 & 7.61\\
&M3 & 27.98 & 26.62 & 27.23 & 24.95 & 23.82 & 22.70 & 20.75 & 19.80 & 19.07 & 18.20 & 18.01 & 16.61 & 13.58 & 11.06 & 11.05 & 10.24 & 8.93 & 8.33 & 8.21 & 7.59\\
&M4 & 28.12 & 26.31 & 26.96 & 24.30 & 22.79 & 21.80 & 19.85 & 18.75 & 18.31 & 17.09 & 16.08 & 15.20 & 12.12 & 10.62 & 10.80 & 8.91 & 8.71 & 7.93 & 7.90 & 7.12\\
&M5 & 27.90 & 26.27 & 26.43 & 23.32 & 22.59 & 21.50 & 19.33 & 17.06 & 17.48 & 14.75 & 14.60 & 12.43 & 11.08 & 9.52 & 8.93 & 8.23 & 8.23 & 7.08 & 7.30 & 6.09\\
&M6 & 27.89 & 25.88 & 25.74 & 22.49 & 20.73 & 19.99 & 16.93 & 14.44 & 14.41 & 12.23 & 9.48 & 9.10 & 7.41 & 5.67 & 4.98 & 4.17 & 3.08 & 2.66 & 2.52 & 2.18\\
\hline
\end{tabular}
\end{center}
}
\end{table*}
%

==> fig/tables/20191209_12564.tex <==
% 20191209_125642
\begin{table*}[t!]
%\small\addtolength{\tabcolsep}{-1pt}
\caption{\label{tab:acc_unit_var_1Q} Accuracy and number of recursions performed statistics for all methods presented in the paper using the setting in \cite{tsiligkaridis2014collaborative}. The evidence distributions are selected as 1D Gaussian distributions with unit variance. Evidence measurement performance is measured with the distance between means of the distributions. Proposed $(T)$ \textbf{(M1)} achieves higher accuracy with lower number of recursions on average with lesser variance.}
{\def\arraystretch{1.5}\tabcolsep=3.5pt
\begin{center}
\tiny
\begin{tabular}{c c c c c c c c c c c c c c c c c c c c c c}
& & \multicolumn{20}{c}{$\delta_\text{means}$} \\
\cline{3-22}
&method &1.5 &1.6 &1.7 &1.8 &1.9 &2 &2.1 &2.2 &2.3 &2.4 &2.5 &2.6 &2.7 &2.8 &2.9 &3 &3.1 &3.2 &3.3 &3.4\\
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Accuracy}}} &M1 & 0.83 & 0.89 & 0.93 & 0.95 & 0.96 & 0.96 & 0.97 & 0.96 & 0.96 & 0.96 & 0.96 & 0.96 & 0.96 & 0.97 & 0.96 & 0.97 & 0.97 & 0.97 & 0.96 & 0.96\\
&M2 & 0.71 & 0.78 & 0.83 & 0.86 & 0.88 & 0.88 & 0.89 & 0.89 & 0.91 & 0.90 & 0.90 & 0.92 & 0.93 & 0.93 & 0.94 & 0.95 & 0.95 & 0.95 & 0.96 & 0.95\\
&M3 & 0.71 & 0.78 & 0.83 & 0.86 & 0.88 & 0.88 & 0.89 & 0.89 & 0.91 & 0.91 & 0.90 & 0.92 & 0.93 & 0.93 & 0.94 & 0.95 & 0.95 & 0.95 & 0.95 & 0.95\\
&M4 & 0.74 & 0.80 & 0.85 & 0.89 & 0.90 & 0.90 & 0.91 & 0.91 & 0.91 & 0.92 & 0.92 & 0.94 & 0.94 & 0.94 & 0.94 & 0.96 & 0.96 & 0.95 & 0.95 & 0.95\\
&M5 & 0.76 & 0.82 & 0.87 & 0.90 & 0.92 & 0.91 & 0.92 & 0.93 & 0.93 & 0.93 & 0.93 & 0.95 & 0.95 & 0.95 & 0.94 & 0.93 & 0.91 & 0.88 & 0.83 & 0.80\\
&M6 & 0.82 & 0.88 & 0.93 & 0.95 & 0.97 & 0.97 & 0.98 & 0.97 & 0.94 & 0.88 & 0.82 & 0.70 & 0.60 & 0.48 & 0.42 & 0.37 & 0.30 & 0.27 & 0.25 & 0.24\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Mean rec.}}} &M1 & 59.25 & 54.48 & 49.50 & 45.30 & 42.09 & 40.31 & 37.05 & 34.74 & 34.13 & 31.99 & 30.86 & 29.88 & 29.56 & 29.13 & 27.45 & 26.90 & 26.32 & 25.90 & 25.50 & 24.93\\
&M2 & 66.16 & 60.81 & 55.65 & 51.41 & 47.70 & 45.59 & 42.12 & 39.52 & 39.21 & 36.75 & 35.29 & 33.36 & 32.86 & 31.64 & 29.63 & 28.63 & 27.95 & 27.37 & 26.89 & 26.28\\
&M3 & 66.09 & 60.77 & 55.62 & 51.37 & 47.62 & 45.55 & 42.01 & 39.47 & 39.12 & 36.71 & 35.23 & 33.33 & 32.80 & 31.62 & 29.59 & 28.59 & 27.88 & 27.34 & 26.84 & 26.23\\
&M4 & 65.07 & 59.52 & 54.39 & 50.07 & 46.52 & 44.45 & 40.77 & 38.23 & 37.93 & 35.41 & 33.92 & 32.32 & 31.65 & 30.66 & 28.73 & 27.93 & 27.08 & 26.60 & 26.10 & 25.38\\
&M5 & 64.14 & 58.62 & 53.33 & 48.87 & 45.36 & 43.24 & 39.59 & 37.13 & 36.54 & 33.78 & 32.39 & 30.98 & 30.37 & 29.55 & 27.64 & 26.92 & 25.98 & 25.36 & 24.68 & 23.86\\
&M6 & 62.46 & 57.04 & 51.75 & 46.90 & 43.16 & 40.80 & 36.73 & 34.14 & 32.72 & 29.62 & 27.39 & 25.22 & 23.53 & 21.65 & 19.91 & 18.53 & 17.51 & 16.69 & 16.04 & 15.39\\
\hline
\hline
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Std. rec.}}} &M1 & 27.82 & 25.86 & 24.03 & 21.95 & 19.97 & 19.02 & 16.52 & 14.76 & 14.52 & 13.07 & 12.45 & 11.35 & 10.94 & 10.37 & 8.93 & 8.87 & 8.12 & 7.54 & 7.40 & 6.91\\
&M2 & 28.02 & 27.08 & 25.96 & 24.47 & 22.89 & 22.25 & 20.36 & 19.13 & 19.27 & 17.83 & 17.25 & 15.25 & 14.44 & 12.58 & 10.84 & 9.78 & 8.90 & 8.27 & 8.02 & 7.53\\
&M3 & 28.02 & 27.06 & 25.94 & 24.45 & 22.83 & 22.23 & 20.29 & 19.10 & 19.19 & 17.79 & 17.21 & 15.25 & 14.37 & 12.59 & 10.82 & 9.76 & 8.84 & 8.25 & 8.01 & 7.50\\
&M4 & 27.92 & 26.75 & 25.48 & 23.82 & 22.18 & 21.45 & 19.34 & 17.99 & 18.15 & 16.68 & 16.03 & 14.20 & 13.34 & 11.88 & 10.17 & 9.41 & 8.35 & 7.86 & 7.65 & 6.92\\
&M5 & 27.82 & 26.51 & 25.14 & 23.25 & 21.53 & 20.79 & 18.43 & 17.15 & 16.90 & 14.97 & 14.37 & 12.72 & 11.80 & 10.88 & 9.08 & 8.83 & 7.75 & 7.05 & 6.76 & 5.97\\
&M6 & 27.80 & 26.25 & 24.66 & 22.56 & 20.34 & 19.39 & 16.25 & 14.50 & 13.68 & 11.83 & 10.26 & 8.75 & 7.44 & 6.03 & 4.81 & 3.81 & 3.19 & 2.65 & 2.51 & 2.24\\
\hline
\end{tabular}
\end{center}
}
\end{table*}
%




==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
